Small-Signal Stability and SCR Enhancement of Offshore WPPs with Synchronous Condensers

Synchronous condensers (SCs) have been reported to improve the overall stability and short-circuit power of a power system. SCs are also being integrated into offshore wind power plants (WPPs) for the same reason. This paper, investigates the effect of synchronous condensers on an offshore wind power plant with grid-following (GFL) and grid-forming (GFM) converter controls. Primarily, the effect of synchronous condensers can be two-fold: (1) overall stability enhancement of the WPP by providing reactive power support, (2) contribution to the effective short circuit ratio (SCR) of the WPP by fault current support. Therefore, this paper focuses on studies concerning these effects on an aggregated model of a WPP connected to the grid. To that end, a state-space model of the test system is developed for small-signal stability assessment and the synchronous condenser's effect on its stability. In addition, a mathematical explanation of SCR enhancement with synchronous condenser is provided and is verified with time-domain electromagnetic transient simulations.

==> bib/Bibliography.tex <==
@article{jia2018assessment,
  title={Assessment of Short Circuit Power and Protection Systems for Future Low Inertia Power Systems.},
  author={Jia, Jundi},
  year={2018},
  publisher={Technical University of Denmark, Department of Electrical Engineering}
}

@INPROCEEDINGS{9449775,
  author={Bao, Li and Fan, Lingling and Miao, Zhixin},
  booktitle={2020 52nd North American Power Symposium (NAPS)}, 
  title={Comparison of Synchronous Condenser and STATCOM for Wind Farms in Weak Grids}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/NAPS50074.2021.9449775}}

@ARTICLE{8742900,
  author={Li, Yin and Fan, Lingling and Miao, Zhixin},
  journal={IEEE Transactions on Power Systems}, 
  title={Wind in Weak Grids: Low-Frequency Oscillations, Subsynchronous Oscillations, and Torsional Interactions}, 
  year={2020},
  volume={35},
  number={1},
  pages={109-118},
  doi={10.1109/TPWRS.2019.2924412}}

@INPROCEEDINGS{6344713,
  author={Huang, Shun-Hsien and Schmall, John and Conto, Jose and Adams, John and Zhang, Yang and Carter, Cathey},
  booktitle={2012 IEEE Power and Energy Society General Meeting}, 
  title={Voltage control challenges on weak grids with high penetration of wind generation: ERCOT experience}, 
  year={2012},
  volume={},
  number={},
  pages={1-7},
  doi={10.1109/PESGM.2012.6344713}}

@INPROCEEDINGS{8601540,
  author={Igbinovia, Famous O. and Fandi, Ghaeth and Muller, Zdenek and Tlusty, Josef},
  booktitle={2018 International Conference on Power System Technology (POWERCON)}, 
  title={Reputation of the Synchronous Condenser Technology in Modern Power Grid}, 
  year={2018},
  volume={},
  number={},
  pages={2108-2115},
  doi={10.1109/POWERCON.2018.8601540}}

@INPROCEEDINGS{5484423,
  author={Marken, Paul E. and Henderson, Mike and LaForest, Dean and Skliutas, John and Roedel, Jim and Campbell, Todd},
  booktitle={IEEE PES T'\&'D 2010}, 
  title={Selection of Synchronous Condenser technology for the Granite Substation}, 
  year={2010},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/TDC.2010.5484423}}

@ARTICLE{7944679,
  author={Fan, Lingling and Miao, Zhixin},
  journal={IEEE Transactions on Sustainable Energy}, 
  title={An Explanation of Oscillations Due to Wind Power Plants Weak Grid Interconnection}, 
  year={2018},
  volume={9},
  number={1},
  pages={488-490},
  doi={10.1109/TSTE.2017.2713980}}

@INPROCEEDINGS{9637902,
  author={Kkuni, Kanakesh Vatta and Nuhic, Mirza and Yang, Guangya},
  booktitle={2021 IEEE Power and Energy Society General Meeting (PESGM)}, 
  title={Power System Stability Impact Assessment for the Current Limits of Grid Supporting Voltage-Source Converters}, 
  year={2021},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/PESGM46819.2021.9637902}}

@ARTICLE{8357471,
  author={Jia, Jundi and Yang, Guangya and Nielsen, Arne Hejde and Rønne-Hansen, Peter},
  journal={IEEE Transactions on Industrial Electronics}, 
  title={Impact of VSC Control Strategies and Incorporation of Synchronous Condensers on Distance Protection Under Unbalanced Faults}, 
  year={2019},
  volume={66},
  number={2},
  pages={1108-1118},
  doi={10.1109/TIE.2018.2835389}}

@INPROCEEDINGS{8905459,
  author={Nuhic, Mirza and Yang, Guangya},
  booktitle={2019 IEEE PES Innovative Smart Grid Technologies Europe (ISGT-Europe)}, 
  title={A Hybrid System Consisting of Synchronous Condenser and Battery - Enhanced Services for Weak Systems}, 
  year={2019},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/ISGTEurope.2019.8905459}}

@INPROCEEDINGS{8443358,
  author={Jia, Jundi and Yang, Guangya and Nielsen, Arne Hejde and Muljadi, Eduard and Weinreich-Jensen, Peter and Gevorgian, Vahan},
  booktitle={2018 5th International Conference on Electric Power and Energy Conversion Systems (EPECS)}, 
  title={Synchronous Condenser Allocation for Improving System Short Circuit Ratio}, 
  year={2018},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/EPECS.2018.8443358}}

@misc{saadat2010power,
  title={Power system analysis},
  author={Saadat, H},
  year={2010, USA: PSA Publishing LLC, Arlington, VA},
  publisher={USA: PSA Publishing LLC, Arlington, VA}
}

@INPROCEEDINGS{898204,
  author={Katsuya, Y. and Mitani, Y. and Tsuji, K.},
  booktitle={PowerCon 2000. 2000 International Conference on Power System Technology. Proceedings (Cat. No.00EX409)}, 
  title={Power system stabilization by synchronous condenser with fast excitation control}, 
  year={2000},
  volume={3},
  number={},
  pages={1563-1568 vol.3},
  doi={10.1109/ICPST.2000.898204}}

@INPROCEEDINGS{7992178,
  author={Hongyang Zhang and Hasler, Jean-Philippe and Johansson, Nicklas and Ängquist, Lennart and Nee, Hans-Peter},
  booktitle={2017 IEEE 3rd International Future Energy Electronics Conference and ECCE Asia (IFEEC 2017 - ECCE Asia)}, 
  title={Frequency response improvement with synchronous condenser and power electronics converters}, 
  year={2017},
  volume={},
  number={},
  pages={1002-1007},
  doi={10.1109/IFEEC.2017.7992178}}

@mastersthesis{ghimire2021dynamics,
  title={Dynamics and Stability of Inverter Dominated Low Inertia Power Grids},
  author={Ghimire, Sulav},
  year={2021},
  school={Skolkovo Institute of Science and Technology, Moscow, Russian Federation}
}

@article{park1929two,
  title={Two-reaction theory of synchronous machines generalized method of analysis-part I},
  author={Park, Robert H},
  journal={Transactions of the American Institute of Electrical Engineers},
  volume={48},
  number={3},
  pages={716--727},
  year={1929},
  publisher={IEEE}
}

@article{Ghimire2023GridForming,
  title={Grid-Forming Control Methods for Weakly Connected Offshore WPPs},
  author={Ghimire, Sulav and Kkuni, Kanakesh V and Jakobsen, Simon C and Knueppel, Thyge and Jensen, Kim H and Guest, Emerson and Rasmussen, Tonny W and Yang, Guangya},
  journal={22nd Wind and Solar Integration Workshop},
  year={2023}
}

@ARTICLE{8412562,
  author={Nguyen, Ha Thi and Yang, Guangya and Nielsen, Arne Hejde and Jensen, Peter Højgaard},
  journal={IEEE Transactions on Sustainable Energy}, 
  title={Combination of Synchronous Condenser and Synthetic Inertia for Frequency Stability Enhancement in Low-Inertia Systems}, 
  year={2019},
  volume={10},
  number={3},
  pages={997-1005},
  doi={10.1109/TSTE.2018.2856938}}

@INPROCEEDINGS{8274566,
  author={Nguyen, Ha Thi and Yang, Guangya and Nielsen, Arne Hejde and Jensen, Peter H⊘jgaard},
  booktitle={2017 IEEE Power and Energy Society General Meeting}, 
  title={Frequency stability enhancement for low inertia systems using synthetic inertia of wind power}, 
  year={2017},
  volume={},
  number={},
  pages={1-5},
  doi={10.1109/PESGM.2017.8274566}}

@INPROCEEDINGS{9020538,
  author={Nguyen, Ha Thi and Guerriero, Cesar and Yang, Guangya and Boltonand, Christopher J and Rahman, Tariq and Jensen, Peter Højgaard},
  booktitle={2019 SoutheastCon}, 
  title={Talega SynCon - Power Grid Support for Renewable-based Systems}, 
  year={2019},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/SoutheastCon42311.2019.9020538}}

@misc{ghosh2023improved,
      title={An Improved Nonlinear Stability Assessment Methodology For Type-4 Wind Turbines via Time Reversal Trajectory}, 
      author={Sujay Ghosh and Mohammad Kazem Bakhshizadeh and Guangya Yang and Łukasz Kocewiak},
      year={2023},
      eprint={2307.11445},
      archivePrefix={arXiv},
      primaryClass={eess.SY}
}

@ARTICLE{653230,
  author={IEEE},
  journal={IEEE Std 1204-1997}, 
  title={IEEE Guide for Planning DC Links Terminating at AC Locations Having Low Short-Circuit Capacities}, 
  year={1997},
  volume={},
  number={},
  pages={1-216},
  doi={10.1109/IEEESTD.1997.85949}}

@techreport{connectionwindfarms,
  type = {Technical Brochures},
  title = {Connection of Wind Farms to Weak AC Networks},
  author = {{Working Group on Wind Farm Connection}},
  year = {2016},
  institution = {CIGRE Study Committee WG B4.62},
  url = {https://e-cigre.org/publication/671-connection-of-wind-farms-to-weak-ac-networks},
}

@ARTICLE{9395086,
  author={Li, Wei and Qian, Ziwei and Wang, Qi and Wang, Yu and Liu, Fusuo and Zhu, Ling and Cheng, Shuo},
  journal={IEEE Access}, 
  title={Transient Voltage Control of Sending-End Wind Farm Using a Synchronous Condenser Under Commutation Failure of HVDC Transmission System}, 
  year={2021},
  volume={9},
  number={},
  pages={54900-54911},
  doi={10.1109/ACCESS.2021.3070979}}

@article{kundur2017power,
  title={Power system dynamics and stability},
  author={Kundur, Prabha S and Balu, Neal J and Lauby, Mark G},
  journal={Power system stability and control},
  volume={3},
  pages={700--701},
  year={2017},
  publisher={McGraw-Hill}
}

@book{miller1982reactive,
  title={Reactive Power Control in Electric Systems},
  author={Miller, Timothy John Eastham},
  year={1982},
  publisher={John Wiley and Sons}
}
